HHH Whitepaper

We here report on the progress of the HHH Workshop, that took place in Dubrovnik in July 2023. After the discovery of a particle that complies with the properties of the Higgs boson of the Standard Model, all Standard Model (SM) parameters are in principle determined. However, in order to verify or falsify the model, the full form of the potential has to be determined. This includes the measurement of the triple and quartic scalar couplings. We here report on ongoing progress of measurements for multi-scalar final states, with an emphasis on three SM-like scalar bosons at 125 GeV, but also mentioning other options. We discuss both experimental progress and challenges as well as theoretical studies and models that can enhance such rates with respect to the SM predictions

==> authors/AuthorAddresses.tex <==
{\footnotesize

\noindent
%$^\ciematno$\ciemat\\ 
$^\essaadino$\essaadi\\
$^\stonybrookno$\stonybrook\\
$^\kitno$\kit\\
$^\boskovicno$\boskovic\\
$^\oxfordno$\oxford\\
$^\ucsdno$\ucsd\\
$^\nikhefno$\nikhef\\
$^\twenteno$\twente\\
$^\ibnzohrno$\ibnzohr\\
$^\iselno$\isel\\
$^\cftcno$\cftc\\
$^\lptheno$\lpthe\\
$^\iitkno$\iitk\\
$^\iceppno$\icepp\\
$^\ufloridano$\uflorida\\
$^\brownno$\brown\\
$^\sfuno$\sfu\\
$^\sysuno$\sysu\\
$^\cernno$\cern\\
$^\ksuno$\ksu\\
$^\lundno$\lund\\
$^\iphtno$\ipht\\
$^\desyno$\desy\\
$^\siegenno$\siegen\\
$^\orsayno$\orsay\\
$^\hamburgno$\hamburg\\
$^\mppno$\mpp\\
$^\tumno$\tum\\
$^\wiscno$\wisc\\
}



==> authors/Authors.tex <==
\begin{center}

\noindent
%Author 1$^\ciematno$,
Hamza Abouabid$^\essaadino$,
Abdesslam Arhrib$^\essaadino$,
Hannah Arnold$^\stonybrookno$,
Duarte Azevedo$^\kitno$,
Vuko Brigljevic $^\boskovicno$,
Maggie Chen $^\oxfordno$,
Daniel Diaz$^\ucsdno$,
Javier Duarte$^\ucsdno$,
Tristan du Pree$^{\nikhefno,\twenteno}$,
Jaouad El Falaki$^{\ibnzohrno}$,
Dinko Ferencek $^\boskovicno$,
Pedro. M. Ferreira $^{\iselno,\cftcno}$,
Benjamin Fuks$^\lptheno$,
Sanmay Ganguly$^{\iitkno,\iceppno}$,
Osama Karkout$^{\nikhefno,\twenteno}$,
Marina Kolosova$^\ufloridano$,
Jacobo Konigsberg$^\ufloridano$,
Greg Landsberg$^\brownno$,
Bingxuan Liu$^{\sfuno,\sysuno}$,
Brian Moser$^\cernno$,
Margarete M\"uhlleitner$^\kitno$,
Andreas Papaefstathiou$^\ksuno$,
Roman Pasechnik$^\lundno$,
Tania Robens$^\boskovicno$,
Rui Santos$^{\iselno,\cftcno}$,
Brian Sheldon$^\ucsdno$,
Gregory Soyez$^\iphtno$,
Marko Stamenkovic$^\brownno$,
Panagiotis Stylianou$^\desyno$,
Tatjana Susa $^\boskovicno$,
Gilberto Tetlalmatzi-Xolocotzi$^{\siegenno,\orsayno}$,
Georg Weiglein$^{\desyno,\hamburgno}$,
Giulia Zanderighi$^{\mppno,\tumno}$,
Rui Zhang$^\wiscno$
%Author 2$^\desyno$
\end{center}

